FLoRA: Enhancing Vision-Language Models with Parameter-Efficient Federated Learning

In the rapidly evolving field of artificial intelligence, multimodal models, e.g., integrating vision and language into visual-language models (VLMs), have become pivotal for many applications, ranging from image captioning to multimodal search engines. Among these models, the Contrastive Language-Image Pre-training (CLIP) model has demonstrated remarkable performance in understanding and generating nuanced relationships between text and images. However, the conventional training of such models often requires centralized aggregation of vast datasets, posing significant privacy and data governance challenges. To address these concerns, this paper proposes a novel approach that leverages Federated Learning and parameter-efficient adapters, i.e., Low-Rank Adaptation (LoRA), to train VLMs. This methodology preserves data privacy by training models across decentralized data sources and ensures model adaptability and efficiency through LoRA's parameter-efficient fine-tuning. Our approach accelerates training time by up to 34.72 times and requires 2.47 times less memory usage than full fine-tuning.

==> content/fig_tex/f03_aircraft.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:aircraft_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:aircraft_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:aircraft_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on FGVCAircraft in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:aircraft}
\end{center}
\end{figure}



==> content/fig_tex/f03_caltech101.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:caltech101_dir}
    \end{subfigure} \hspace{0em}%
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:caltech101_dir05}
    \end{subfigure} \hspace{0em}%
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:caltech101_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Caltech101 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:caltech101}
\end{center}
\end{figure}



==> content/fig_tex/f03_cars.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:cars_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:cars_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:cars_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on StanfordCARS in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:stanfordcars}
\end{center}
\end{figure}



==> content/fig_tex/f03_cifar10.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:cifar10_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:cifar10_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:cifar10_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on CIFAR-10 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:cifar10}
\end{center}
\end{figure}



==> content/fig_tex/f03_cifar100.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:cifar100_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:cifar100_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:cifar100_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on CIFAR-100 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:cifar100}
\end{center}
\end{figure}



==> content/fig_tex/f03_country211.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:country211_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:country211_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:country211_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Country211 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:country211}
\end{center}
\end{figure}



==> content/fig_tex/f03_dtd.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:dtd_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:dtd_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:dtd_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on DTD in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:dtd}
\end{center}
\end{figure}



==> content/fig_tex/f03_eurosat.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:eurosat_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:eurosat_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:eurosat_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on EuroSAT in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:eurosat}
\end{center}
\end{figure}



==> content/fig_tex/f03_fer2013.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:fer2013_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:fer2013_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:fer2013_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on FER2013 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:fer2013}
\end{center}
\end{figure}



==> content/fig_tex/f03_flowers.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:flowers_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:flowers_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:flowers_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Oxford 102 Flower in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:oxfordflowers}
\end{center}
\end{figure}



==> content/fig_tex/f03_fmnist.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:fmnist_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:fmnist_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:fmnist_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Fashion-MNIST in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:fmnist}
\end{center}
\end{figure}



==> content/fig_tex/f03_food101.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:food101_sub1}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:food101_sub2}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:food101_sub3}
    \end{subfigure}
    \caption{The data distribution of all clients on Food101 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:food101}
\end{center}
\end{figure}



==> content/fig_tex/f03_iid.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.240\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_iid.pdf}
        \caption{F-MNIST}
        \label{fig:fmnist_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.240\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_iid.pdf}
        \caption{CIFAR-10}
        \label{fig:cifar10_iid}
    \end{subfigure}
    \begin{subfigure}[b]{0.240\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_iid.pdf}
        \caption{EuroSAT}
        \label{fig:eurosat_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.240\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_iid.pdf}
        \caption{FER2013}
        \label{fig:fer2013_iid}
    \end{subfigure}

    \vspace{0.5em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_iid.pdf}
        \caption{CIFAR-100}
        \label{fig:cifar100_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_iid.pdf}
        \caption{Food101}
        \label{fig:food101_iid}
    \end{subfigure}

    \vspace{0.5em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_iid.pdf}
        \caption{OxfordPETS}
        \label{fig:pets_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_iid.pdf}
        \caption{DTD}
        \label{fig:dtd_iid}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_iid.pdf}
        \caption{SST2}
        \label{fig:sst2_iid}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.240\linewidth}
    %     \includegraphics[width=\linewidth]{content/fig/pcam_iid.pdf}
    %     \caption{PCAM}
    %     \label{fig:pcam_iid}
    % \end{subfigure}

    \vspace{0.5em} % Adjust the vertical space between rows
    
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_iid.pdf}
        \caption{Flowers102}
        \label{fig:flowers_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_iid.pdf}
        \caption{FGVCAircraft}
        \label{fig:aircraft_iid}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_iid.pdf}
        \caption{Caltech101}
        \label{fig:caltech101_iid}
    \end{subfigure}

    \vspace{0.5em} % Adjust the vertical space between rows
    
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_iid.pdf}
        \caption{Tiny-ImageNet}
        \label{fig:tiny_iid}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_iid.pdf}
        \caption{StanfordCARS}
        \label{fig:cars_iid}
    \end{subfigure}
    
    % \begin{subfigure}[b]{\linewidth}
    %     \includegraphics[width=\linewidth]{content/fig/DomainNet_iid.pdf}
    %     \caption{DomainNet}
    %     \label{fig:DomainNet_iid}
    % \end{subfigure} \hspace{0em}%

    \vspace{0.5em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_iid.pdf}
        \caption{Country211}
        \label{fig:country211_iid}
    \end{subfigure}
    
    \vspace{0.5em} % Adjust the vertical space between rows
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_iid.pdf}
        \caption{SUN397}
        \label{fig:sun397_iid}
    \end{subfigure}
    
    \caption{The data distribution of all clients on different datasets in IID settings. The size of a circle means the number of data samples.}
    \label{fig:iid}
\end{center}
\end{figure}



==> content/fig_tex/f03_pets.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:pets_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:pets_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:pets_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Oxford-IIIT Pet in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:oxfordpets}
\end{center}
\end{figure}



==> content/fig_tex/f03_sst2.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:sst2_dir}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:sst2_dir05}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:sst2_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Rendered SST2 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:sst2}
\end{center}
\end{figure}



==> content/fig_tex/f03_sun397.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:sun397_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:sun397_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:sun397_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on SUN397 in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:sun397}
\end{center}
\end{figure}



==> content/fig_tex/f03_tiny.tex <==
\begin{figure}[ht]
\begin{center}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_dir.pdf}
        \caption{$\beta = 0.1$}
        \label{fig:tiny_dir}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_dir05.pdf}
        \caption{$\beta = 0.5$}
        \label{fig:tiny_dir05}
    \end{subfigure} 
    \vspace{0em}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_dir10.pdf}
        \caption{$\beta = 1.0$}
        \label{fig:tiny_dir10}
    \end{subfigure}
    \caption{The data distribution of all clients on Tiny-ImageNet in practical settings with varying $\beta$. The size of a circle means the number of data samples.}
    \label{fig:tiny}
\end{center}
\end{figure}



==> content/fig_tex/f04_fs_iid.tex <==
\begin{figure*}[ht]
\begin{center}

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_iid_fs.pdf}
        \label{fig:fmnist_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_iid_fs.pdf}
        \label{fig:cifar10_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_iid_fs.pdf}
        \label{fig:cifar100_iid_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_iid_fs.pdf}
        \label{fig:tiny_iid_fs}
    \end{subfigure} \hspace{0em}%
    
    \vspace{0.0em} % Adjust the vertical space between rows
    
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_iid_fs.pdf}
        \label{fig:pets_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_iid_fs.pdf}
        \label{fig:flowers_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_iid_fs.pdf}
        \label{fig:aircraft_iid_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_iid_fs.pdf}
        \label{fig:cars_iid_fs}
    \end{subfigure}

    \vspace{0.0em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_iid_fs.pdf}
        \label{fig:dtd_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_iid_fs.pdf}
        \label{fig:eurosat_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_iid_fs.pdf}
        \label{fig:fer2013_iid_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_iid_fs.pdf}
        \label{fig:caltech101_iid_fs}
    \end{subfigure}

    \vspace{0.0em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_iid_fs.pdf}
        \label{fig:food101_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_iid_fs.pdf}
        \label{fig:country211_iid_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_iid_fs.pdf}
        \label{fig:sun397_iid_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_iid_fs.pdf}
        \label{fig:sst2_iid_fs}
    \end{subfigure} \hspace{0em}%
    
    \caption{Results of few-shot learning on various datasets with IID setting.}
    \label{fig:fs_iid}
    
\end{center}
\end{figure*}

==> content/fig_tex/f04_fs_pat.tex <==
\begin{figure*}[ht]
\begin{center}

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fmnist_pat_fs.pdf}
        \label{fig:fmnist_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar10_pat_fs.pdf}
        \label{fig:cifar10_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cifar100_pat_fs.pdf}
        \label{fig:cifar100_pat_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/tiny_pat_fs.pdf}
        \label{fig:tiny_pat_fs}
    \end{subfigure} \hspace{0em}%
    
    \vspace{0.0em} % Adjust the vertical space between rows
    
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/pets_pat_fs.pdf}
        \label{fig:pets_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/flowers_pat_fs.pdf}
        \label{fig:flowers_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/aircraft_pat_fs.pdf}
        \label{fig:aircraft_pat_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/cars_pat_fs.pdf}
        \label{fig:cars_pat_fs}
    \end{subfigure}

    \vspace{0.0em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/dtd_pat_fs.pdf}
        \label{fig:dtd_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/eurosat_pat_fs.pdf}
        \label{fig:eurosat_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/fer2013_pat_fs.pdf}
        \label{fig:fer2013_pat_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/caltech101_pat_fs.pdf}
        \label{fig:caltech101_pat_fs}
    \end{subfigure}

    \vspace{0.0em} % Adjust the vertical space between rows

    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/food101_pat_fs.pdf}
        \label{fig:food101_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/country211_pat_fs.pdf}
        \label{fig:country211_pat_fs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sun397_pat_fs.pdf}
        \label{fig:sun397_pat_fs}
    \end{subfigure} \hspace{0em}%
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \includegraphics[width=\linewidth]{content/fig/sst2_pat_fs.pdf}
        \label{fig:sst2_pat_fs}
    \end{subfigure} \hspace{0em}%
    
    \caption{Results of few-shot learning on various datasets with pathological non-IID setting.}
    \label{fig:fs_pat}
\end{center}
\end{figure*}

==> content/tab_tex/t01_iid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{The accuracy (\%) of the image classification tasks for IID.}
\label{tab:iid}
\begin{center}
\begin{tabular}{c|cccccccccccc}
\toprule
& \multicolumn{12}{|c}{\textbf{IID}} \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Dataset}} & 
\multicolumn{1}{c} {FMNIST} & 
\multicolumn{1}{c} {CIFAR10} & 
\multicolumn{1}{c} {CIFAR100} &  
\multicolumn{1}{c} {DIGIT5} & 
\multicolumn{1}{c} {TINY} & 
\multicolumn{1}{c} {PETS} & 
\multicolumn{1}{c} {FLOWERS} & 
\multicolumn{1}{c} {AIRCRAFT} & 
\multicolumn{1}{c} {FOOD} & 
\multicolumn{1}{c} {DomainNet} &
\multicolumn{1}{c} {COUNTRY} & 
\multicolumn{1}{c} {SUN} \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Clients}} & $N = 10$ & $N = 10$ & $N = 10$ & $N = 5$ & $N = 10$ & $N = 10$ & $N = 10$ & $N = 10$ & $N = 10$ & $N = 6$ & $N = 10$ & $N = 10$ \\ 
\midrule
\textbf{Local}      & - & - & - & - & - & - & - & - & - & - \\

\textbf{FFT}        & 76.76 & 88.28 & 61.85 & 29.55 & 60.05 & 82.03 & 63.12 & 19.49 & - & - \\

\textbf{LC}         & 78.84 & \textbf{98.25} & 47.20 & 61.39 & 42.12 & 39.24 & 19.00 & 4.71 & - & - \\

\textbf{VM-LC}      & 75.55 & 85.78 & 46.02 & \textbf{88.37} & 21.02 & 46.60 & 27.55 & 5.89 & - & - \\

\textbf{AA}         & 81.08 & 91.99 & 66.83 & 55.45 & 63.17 & 85.22 & 68.03 & 23.27 & - & - \\
\midrule
\textbf{Ours}       & \textbf{89.81} & 92.26 & \textbf{78.70} & 76.79 & \textbf{73.93} & \textbf{91.87} & \textbf{95.69} & \textbf{45.42} & - & -  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t02_pat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{The test accuracy (\%) of the image classification tasks for pathological non-IID with $N = 10$.}
\label{tab:pat}
\begin{center}
\begin{tabular}{c|ccccccccccc}
\toprule
% \multicolumn{1}{c|}{\boldmath{$N = 10$}} & \multicolumn{10}{c}{\textbf{Pathological label skew non-IID}} \\ 
% \midrule
\multicolumn{1}{c|}{\textbf{Dataset}} & \multicolumn{1}{|c} {FMNIST} & 
\multicolumn{1}{c} {CIFAR10} & 
\multicolumn{1}{c} {CIFAR100} & 
\multicolumn{1}{c} {TINY} & 
\multicolumn{1}{c} {PETS} & 
\multicolumn{1}{c} {FLOWERS} & 
\multicolumn{1}{c} {AIRCRAFT} & 
\multicolumn{1}{c} {FOOD} & 
\multicolumn{1}{c} {COUNTRY} & 
\multicolumn{1}{c} {SUN} &
\multicolumn{1}{c} {SST2} \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Class per client}} & $2$ & $2$ & $20$ & $40$ & $7$ & $20$ & $20$ & $20$ & $42$ & $79$ & $1$ \\ 
\midrule
\textbf{Local}          & - & - & - & - & - & - & - & - \\

\textbf{FedFFT}         & 92.21 & 88.28 & \textbf{76.66} & 61.90 & - & - & 18.63 & - \\

\textbf{FedLC}          & \textbf{98.59} & \textbf{98.24} & 75.01 & 61.38 & - & - & \textbf{39.19} & - \\

\textbf{FedVM-LC}       & 98.15 & 83.52 & 24.98 & 8.41 & - & - & 32.51 & - \\

\textbf{FedAA}          & 64.17 & 92.02 & 66.19 & 62.86 & - & - & 23.63 & - \\
\midrule
\textbf{Ours}           & 72.74 & 92.31 & 73.20 & \textbf{71.03} & - & - & 34.52 & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t03_prac.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{The test accuracy (\%) of the image classification tasks for practical non-IID.}
\label{tab:prac}
\begin{center}
\begin{tabular}{c|ccccccccccccccc}
\toprule
% & \multicolumn{13}{|c}{\textbf{Practical label skew non-IID}} \\ 
% \midrule
\multicolumn{1}{c|}{\textbf{Dataset}} & \multicolumn{1}{c} {FMNIST} & \multicolumn{1}{c} {CIFAR10} & \multicolumn{1}{c} {CIFAR100} & \multicolumn{2}{c} {TINY} & \multicolumn{2}{c} {PETS} & \multicolumn{2}{c} {FLOWERS} & \multicolumn{2}{c} {AIRCRAFT} & \multicolumn{2}{c} {COUNTRY}\\ 
\midrule
\multicolumn{1}{c|}{\boldmath{$N = 10$}} & $\beta = 0.1$ & $\beta = 0.1$ & $\beta = 0.1$ & $\beta = 0.1$ & $\beta = 0.5$ & $\beta = 0.1$ & $\beta = 0.5$ & $\beta = 0.1$ & $\beta = 0.5$ & $\beta = 0.1$ & $\beta = 0.5$ & $\beta = 0.1$ & $\beta = 0.5$ \\ 
\midrule
\textbf{Local}      & - & - & - & - & - & - & - & - & - & - & - & - \\

\textbf{FFT}        & 82.80 & - & 69.20 & 64.14 & - & 81.56 & 81.72 & 74.75 & 79.33 & 18.49 & 18.15 \\

\textbf{LC}         & \textbf{96.38} & - & 63.08 & 56.11 & - & 78.42 & 49.91 & 70.89 & 48.22 & \textbf{44.31} & 22.48 \\

\textbf{VM-LC}      & 94.28 & - & 26.97 & 11.08 & - & 75.48 & 48.01 & 67.21 & 49.53 & 42.17 & 20.41 \\

\textbf{AA}         & 69.72 & - & 65.54 & 61.93 & - & 78.32 & 82.49 & 62.43 & 67.32 & 22.75 & 21.34 \\
\midrule
\textbf{Ours}       & 81.04 & - & \textbf{75.33} & \textbf{71.23} & - & \textbf{88.91} & \textbf{90.14} & \textbf{91.97} & \textbf{95.65} & 40.48 & \textbf{43.48} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t05_comm_lc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table}[ht]
\caption{ The communication overhead on FLOWERS dataset for LC and VM-LC (per iteration).}
\label{tab:communication_lc}
\begin{center}
\begin{tabular}{c|cc|cc}
\toprule
& \multicolumn{2}{|c}{\textbf{Number of Parameters}} & \multicolumn{2}{|c}{\textbf{Size (MB)}} \\ 
\midrule
& \multicolumn{1}{c}{FedLC} & \multicolumn{1}{c}{FedVM-LC} & \multicolumn{1}{|c}{FedLC} & \multicolumn{1}{c}{FedVM-LC} \\ 
\midrule
{F-MNIST}       & 5,130 & 87,461,130 & 0.020 & 333.638 \\

{CIFAR-10}      & 5,130 & 87,461,130 & 0.020 & 333.638 \\

{CIFAR-100}     & 51,300 & 87,507,300 & 0.196 & 333.814 \\

{TINY}          & 102,600 & 87,558,600 & 0.391 & 334.010 \\

{OxfordPets}    & 8,981 & 87,474,981 & 0.072 & 333.691 \\

{Flowers102}    & 52,326 & 87,508,326 & 0.200 & 333.818 \\

{Aircraft}      & 51,300 & 87,507,300 & 0.196 & 333.814 \\

{Cars}          & 100,548 & 87,556,548 & 0.387 & 334.002 \\

{DTD}           & 24,111 & 87,480,111 & 0.092 & 333.711 \\

{EuroSAT}       & 5,130 & 87,461,130 & 0.020 & 333.638 \\

{FER2013}       & 3,591 & 87,459,591 & 0.014 & 333.632 \\

{Caltech101}    & 51,813 & 87,507,813 & 0.198 & 333.816 \\

{Food101}       & 51,813 & 87,507,813 & 0.198 & 333.816 \\

{Country211}    & 108,243 & 87,564,243 & 0.413 & 334.031 \\

{SUN397}        & 203,661 & 87,659,661 & 0.777 & 334.395 \\

{R-SST2}          & 1,026 & 87,457,026 & 0.004 & 333.622 \\

\bottomrule
\end{tabular}

\vspace{-2.0em}

\end{center}
\end{table}


==> content/tab_tex/t05_overhead.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{ The computation and communication overhead on FLOWERS dataset (per iteration) (IID).}
\label{tab:overhead}
\begin{center}
\begin{tabular}{c|ccc|cc}
\toprule
& \multicolumn{3}{|c|}{\textbf{Computation}} & \multicolumn{2}{|c}{\textbf{Communication}} \\ 
\midrule
& \multicolumn{1}{|c}{Total time (min)} & \multicolumn{1}{c}{Average time (s)} & \multicolumn{1}{c|}{Memory (GB)} & \multicolumn{1}{c}{Number of Parameters} & \multicolumn{1}{c}{Size (MB)} \\ 
\midrule
\textbf{FedFFT}     & 89.07 & 5,329.55 & 29.76 & 151,277,313 & 577,078 \\

\textbf{FedLC}      & 73.33 & 4,394.76 & 10.90 & 52,326 & 0.200 \\

\textbf{FedVM-LC}   & 79.20 & 4,743.1 & 23.44 & 87,462,156 & 333,818 \\

\textbf{FedAA}      & 77.52 & 4,645.05 &  11.03 & 525,312 & 2.004 \\

\midrule

\textbf{Ours}       & 83.52 & 5,006.86 & 11.90 & 196,608 & 0.751 \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t06_stability_dir.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table}[ht]
\caption{The test accuracy (\%) of the methods on  with $N = 10$,  $\beta= 0.1$, and $\rho \le 1$.}
\label{tab:stability_dir}
\begin{center}
\begin{tabular}{c|ccc}
\toprule
& \multicolumn{1}{|c}{$\rho = 1$} & \multicolumn{1}{c}{$\rho \in [0.5, 1]$} & \multicolumn{1}{c}{$\rho \in [0.1, 1]$} \\ 
\midrule
\textbf{FedFFT}     & - & - & - \\

\textbf{FedLC}      & - & - & - \\

\textbf{FedVM-LC}   & - & - & - \\

\textbf{FedAA}   & - & - & - \\

\midrule

\textbf{Ours}   & - & - & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> content/tab_tex/t06_stability_dir_vertical.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table}[ht]
\caption{The test accuracy (\%) of the methods on  with $N = 10$,  $\beta= 0.1$, and $\rho \le 1$ (robustness).}
\label{tab:stability_dir_vertical}
\begin{center}
\begin{tabular}{c|c|cccc|c}
\toprule
\multicolumn{1}{c} {\textbf{Dataset}} & \multicolumn{1}{|c|} {\boldmath{$\rho$}} & \textbf{FFT} & \textbf{LC} & \textbf{VM-LC} & \textbf{AA} & \textbf{Ours} \\
\midrule

\multirow{2}{*} {F-MNIST}        
                                & $[0.5, 1]$ & 82.92 & \cellcolor{blue!25} \textbf{96.21} & 94.35 & 69.66 & 81.55 \\
                                & $[0.1, 1]$ & 81.94 & \cellcolor{blue!25} \textbf{96.35} & 95.07 & 69.87 & 82.55 \\
\midrule  

\multirow{2}{*} {CIFAR-10}       
                                & $[0.5, 1]$ & 87.04 & 92.36 & 82.20 & 89.77 & \cellcolor{blue!25} \textbf{92.51} \\
                                & $[0.1, 1]$ & 87.04 & 91.70 & 82.19 & 90.03 & \cellcolor{blue!25} \textbf{92.71} \\
\midrule  

\multirow{2}{*} {CIFAR-100}      
                                & $[0.5, 1]$ & 71.34 & 61.87 & 26.31 & 65.46 & \cellcolor{blue!25} \textbf{75.38} \\
                                & $[0.1, 1]$ & 68.71 & 60.61 & 25.50 & 65.01 & \cellcolor{blue!25} \textbf{74.64} \\
\midrule 

\multirow{2}{*} {TINY}          
                                & $[0.5, 1]$ & 62.78 & 55.58 & 10.83 & 61.84 & \cellcolor{blue!25} \textbf{71.26} \\
                                & $[0.1, 1]$ & 64.78 & 55.44 & 10.69 & 61.48 & \cellcolor{blue!25} \textbf{70.62} \\
\midrule    

\multirow{2}{*} {OxfordPets}          
                                & $[0.5, 1]$ & 81.56 & 74.98 & 75.33 & 78.30 & \cellcolor{blue!25} \textbf{88.87} \\
                                & $[0.1, 1]$ & 81.56 & 78.30 & 69.02 & 78.09 & \cellcolor{blue!25} \textbf{88.70} \\
\midrule    

\multirow{2}{*} {Flowers102}       
                                & $[0.5, 1]$ & 81.23 & 70.53 & 69.94 & 66.70 &  \cellcolor{blue!25} \textbf{93.93} \\
                                & $[0.1, 1]$ & 78.79 & 70.88 & 63.97 & 65.78 & \cellcolor{blue!25} \textbf{92.96} \\
\midrule  

\multirow{2}{*} {Aircraft}      
                                & $[0.5, 1]$ & 18.51 & \cellcolor{blue!25} \textbf{44.11} & 33.98 & 21.74 & 41.50 \\
                                & $[0.1, 1]$ & 18.75 & \cellcolor{blue!25} \textbf{43.25} & 37.87 & 21.11 & 39.32 \\
\midrule  

\multirow{2}{*} {Cars}          
                                & $[0.5, 1]$ & 47.14 & 58.92 & 49.06 & 51.67 & \cellcolor{blue!25} \textbf{72.74} \\
                                & $[0.1, 1]$ & 47.14  & 58.60 & 45.77 & 50.35 & \cellcolor{blue!25} \textbf{72.75} \\

\midrule 

\multirow{2}{*} {DTD}          
                                & $[0.5, 1]$ & 75.94 & \cellcolor{blue!25} \textbf{76.82} & 75.94 & 44.97 & 67.96 \\
                                & $[0.1, 1]$ & 74.28 & \cellcolor{blue!25} \textbf{76.84} & 71.34 & 43.74 & 68.48 \\

\midrule 

\multirow{2}{*} {EuroSAT}          
                                & $[0.5, 1]$ & 80.77 & 87.83 & \cellcolor{blue!25} \textbf{92.59} & 58.03 & 89.11 \\
                                & $[0.1, 1]$ & 86.19 & 86.48 & \cellcolor{blue!25} \textbf{90.51} & 56.65 & 88.98 \\

\midrule 

\multirow{2}{*} {FER2013}          
                                & $[0.5, 1]$ & 41.88 & 91.91 & \cellcolor{blue!25} \textbf{91.98} & 32.85 & 43.31 \\
                                & $[0.1, 1]$ & 45.96 & \cellcolor{blue!25} \textbf{91.60} & 91.01 & 29.44 & 51.98 \\

\midrule 

\multirow{2}{*} {Caltech101}          
                                & $[0.5, 1]$ & 88.70 & 87.31 & 86.54 & 88.22 & \cellcolor{blue!25} \textbf{94.46} \\
                                & $[0.1, 1]$ & 89.49 & 87.01 & 85.48 & 88.11 & \cellcolor{blue!25} \textbf{94.67} \\

\midrule 

\multirow{2}{*} {Food101}       
                                & $[0.5, 1]$ & 79.46 & 70.36 & 16.34 & 79.00 & \cellcolor{blue!25} \textbf{81.75} \\
                                & $[0.1, 1]$ & 79.46 & 69.93 & 15.72 & 78.83 & \cellcolor{blue!25} \textbf{81.67} \\
\midrule 

\multirow{2}{*} {Country211}       & $[0.5, 1]$ & 17.27 & \cellcolor{blue!25} \textbf{27.88} & 5.37 & 15.67 & 24.74 \\
                                & $[0.1, 1]$ & 16.78 & \cellcolor{blue!25} \textbf{27.54} & 5.09 & 14.64 & 22.59 \\
\midrule 

\multirow{2}{*} {SUN397}        
                                & $[0.5, 1]$ & 60.94 & 63.33 & 16.24 & 61.84 & \cellcolor{blue!25} \textbf{71.66} \\
                                & $[0.1, 1]$ & 61.21 & 63.10 & 15.86 & 61.71 & \cellcolor{blue!25} \textbf{71.94} \\
\midrule 

\multirow{2}{*} {SST2}          
                                & $[0.5, 1]$ & 58.01 & \cellcolor{blue!25} \textbf{99.20} & \cellcolor{blue!25} \textbf{99.20} & 55.09 & 71.27 \\
                                & $[0.1, 1]$ & 59.20 & \cellcolor{blue!25} \textbf{99.20} & \cellcolor{blue!25} \textbf{99.20} & 54.97 & 72.01 \\

% \midrule  

% \multirow{2}{*} {PCAM}          
%                                 & $[0.5, 1]$ & - & - & - & - & - \\
%                                 & $[0.1, 1]$ & - & - & - & - & - \\
                                
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> content/tab_tex/t06_stability_iid_vertical.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table}[ht]
\caption{The test accuracy (\%) of the methods on  with $N = 10$, IID, and $\rho \le 1$ (robustness).}
\label{tab:stability_iid_vertical}
\begin{center}
\begin{tabular}{c|c|cccc|c}
\toprule
\multicolumn{1}{c} {\textbf{Dataset}} & \multicolumn{1}{|c|} {\boldmath{$\rho$}} & \textbf{FFT} & \textbf{LC} & \textbf{VM-LC} & \textbf{AA} & \textbf{Ours} \\
\midrule

\multirow{2}{*} {F-MNIST}        
                                & $[0.5, 1]$ & 68.50 & 78.35 & 62.46 & 80.96 & \cellcolor{blue!25} \textbf{89.85} \\
                                & $[0.1, 1]$ & 67.90 & 78.08 & 57.87 & 80.84 & \cellcolor{blue!25} \textbf{89.74} \\
\midrule  

\multirow{2}{*} {CIFAR-10}       
                                & $[0.5, 1]$ & 88.19 & 88.25 & 80.69 & 89.35 & \cellcolor{blue!25} \textbf{94.76} \\
                                & $[0.1, 1]$ & 88.19 & 87.96 & 72.88 & 88.78 & \cellcolor{blue!25} \textbf{94.70} \\
\midrule  

\multirow{2}{*} {CIFAR-100}      
                                & $[0.5, 1]$ & 61.85 & 46.98 & 47.22 & 66.74 & \cellcolor{blue!25} \textbf{78.65} \\
                                & $[0.1, 1]$ & 61.88 & 47.24 & 36.08 & 66.37 & \cellcolor{blue!25} \textbf{78.32} \\
\midrule 

\multirow{2}{*} {TINY}          
                                & $[0.5, 1]$ & 60.05 & 41.82 & 28.48 & 62.94 & \cellcolor{blue!25} \textbf{73.71} \\
                                & $[0.1, 1]$ & 60.05 & 41.67 & 13.17 & 62.72 & \cellcolor{blue!25} \textbf{73.65} \\
\midrule    

\multirow{2}{*} {OxfordPets}          
                                & $[0.5, 1]$ & 82.03 & 33.06 & 45.75 & 84.52 & \cellcolor{blue!25} \textbf{91.82} \\
                                & $[0.1, 1]$ & 82.03 & 29.43 & 44.48 & 83.60 & \cellcolor{blue!25} \textbf{91.37} \\
\midrule    

\multirow{2}{*} {Flowers102}       
                                & $[0.5, 1]$ & 64.86 & 16.66 & 30.47 & 69.57 & \cellcolor{blue!25} \textbf{96.70} \\
                                & $[0.1, 1]$ & 72.36 & 16.27 & 29.97 & 67.63 & \cellcolor{blue!25} \textbf{96.32} \\
\midrule  

\multirow{2}{*} {Aircraft}      
                                & $[0.5, 1]$ & 18.96 & 7.0 & 7.32 & 21.36 & \cellcolor{blue!25} \textbf{48.56} \\
                                & $[0.1, 1]$ & 18.96 & 6.72 & 8.32 & 21.44 & \cellcolor{blue!25} \textbf{49.32} \\
\midrule  

\multirow{2}{*} {Cars}          
                                & $[0.5, 1]$ & 48.95 & 9.26 & 9.36 & 52.86 & \cellcolor{blue!25} \textbf{79.69} \\
                                & $[0.1, 1]$ & 48.95 & 9.30 & 9.95 & 52.39 & \cellcolor{blue!25} \textbf{79.12} \\

\midrule  

\multirow{2}{*} {DTD}          
                                & $[0.5, 1]$ & 54.60 & 39.00 & 42.26 & 43.12 & \cellcolor{blue!25} \textbf{74.82} \\
                                & $[0.1, 1]$ & 56.38 & 36.95 & 41.84 & 42.26 & \cellcolor{blue!25} \textbf{75.60} \\

\midrule  

\multirow{2}{*} {EuroSAT}          
                                & $[0.5, 1]$ & 84.22 & 77.80 & 81.11 & 82.47 & \cellcolor{blue!25} \textbf{95.18} \\
                                & $[0.1, 1]$ & 86.50 & 76.08 & 80.54 & 81.92 & \cellcolor{blue!25} \textbf{95.21} \\

\midrule  

\multirow{2}{*} {FER2013}          
                                & $[0.5, 1]$ & 40.21 & 47.14 & 44.91 & 56.97 & \cellcolor{blue!25} \textbf{66.24} \\
                                & $[0.1, 1]$ & 40.21 & 39.28 & 42.14 & 56.44 & \cellcolor{blue!25} \textbf{66.14} \\

\midrule  

\multirow{2}{*} {Caltech101}          
                                & $[0.5, 1]$ & 88.58 & 51.14 & 49.99 & 89.45 & \cellcolor{blue!25} \textbf{95.99} \\
                                & $[0.1, 1]$ & 88.40 & 52.47 & 50.53 & 89.18 & \cellcolor{blue!25} \textbf{95.60} \\

\midrule 

\multirow{2}{*} {Food101}       
                                & $[0.5, 1]$ & 79.71 & 63.96 & 38.82 & 79.97 & \cellcolor{blue!25} \textbf{84.09} \\
                                & $[0.1, 1]$ & 79.71 & 63.77 & 17.2 & 79.94 & \cellcolor{blue!25} \textbf{83.95} \\
\midrule 

\multirow{2}{*} {Country211}    
                                & $[0.5, 1]$ & 15.66 & 7.80 & 4.94 & 15.45 & \cellcolor{blue!25} \textbf{25.04} \\
                                & $[0.1, 1]$ & 15.66 & 7.58 & 2.93 & 15.28 & \cellcolor{blue!25} \textbf{25.31} \\
\midrule 

\multirow{2}{*} {SUN397}        
                                & $[0.5, 1]$ & 58.99 & 26.81 & 15.55 & 61.48 & \cellcolor{blue!25} \textbf{76.29} \\
                                & $[0.1, 1]$ & 58.99 & 25.84 & 12.21 & 61.33 & \cellcolor{blue!25} \textbf{76.34} \\
\midrule 

\multirow{2}{*} {SST2}          
                                & $[0.5, 1]$ & 60.62 & 64.89 & 60.33 & 63.23 & \cellcolor{blue!25} \textbf{70.49} \\
                                & $[0.1, 1]$ & 60.62 & 64.10 & 59.33 & 62.32 & \cellcolor{blue!25} \textbf{70.37} \\

% \midrule 

% \multirow{2}{*} {PCAM}          
%                                 & $[0.5, 1]$ & - & - & - & - & - \\
%                                 & $[0.1, 1]$ & - & - & - & - & - \\
                                
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> content/tab_tex/t08_hyper.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{Different configurations of LoRA within CLIP on FLOWERS dataset.}
\label{tab:hyper}
\begin{center}
\begin{tabular}{c|cccccc|cccccc}
\toprule
% & \multicolumn{12}{|c}{\textbf{LoRA configuration}} \\ 
% \midrule
\multicolumn{1}{c|}{\textbf{Hyperparameter}} & \multicolumn{6}{|c} {\textbf{Rank}} & \multicolumn{6}{c} {\textbf{Scaling factor}}  \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Value}} & r = 1 & \cellcolor{blue!25} r = 2 & r = 4 & r = 8 & r = 16 & r = 32 & $\alpha$ = 1 & $\alpha$ = 4 & $\alpha$ = 8 & $\alpha$ = 16 & \cellcolor{blue!25}  $\alpha$ = 32 & $\alpha$ = 64 \\ 
\midrule
\textbf{Accuracy}    & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t08_hyper_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{Different configurations of LoRA within CLIP on different dataset.}
\label{tab:hyper_new}
\begin{center}
\begin{tabular}{c|cccccc|cccccc}
\toprule
% & \multicolumn{12}{|c}{\textbf{LoRA configuration}} \\ 
% \midrule
\multicolumn{1}{c|}{\textbf{Hyperparameter}} & \multicolumn{6}{c} {\textbf{OxfordPets}} & \multicolumn{6}{c} {\textbf{FLowers102}}  \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Scaling factor}} & \multicolumn{12}{c} 32 \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Value}} & r = 1 & \cellcolor{blue!25} r = 2 & r = 4 & r = 8 & r = 16 & r = 32 & $\alpha$ = 1 & $\alpha$ = 4 & $\alpha$ = 8 & $\alpha$ = 16 & \cellcolor{blue!25}  $\alpha$ = 32 & $\alpha$ = 64 \\ 
\midrule
\textbf{Accuracy}    & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> content/tab_tex/t09_position.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{booktabs} % For formal tables
\begin{table*}[ht]
\caption{Different positions of LoRA within CLIP on FLOWERS dataset.}
\label{tab:position}
\begin{center}
\begin{tabular}{c|cccccccccccc|cccccccccccc}
\toprule
& \multicolumn{12}{|c}{\textbf{Text Encoder}} & \multicolumn{12}{|c}{\textbf{Image Encoder}} \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Block}} & \multicolumn{2}{|c} {Query} & \multicolumn{2}{c} {Key} & \multicolumn{2}{c} {Value} & \multicolumn{2}{c} {Projection} & \multicolumn{2}{c} {MLP} & \multicolumn{2}{c} {Head} & \multicolumn{2}{|c} {Query} & \multicolumn{2}{c} {Key} & \multicolumn{2}{c} {Value} & \multicolumn{2}{c} {Projection} & \multicolumn{2}{c} {MLP} & \multicolumn{2}{c} {Head} \\ 
\midrule
\multicolumn{1}{c|}{\textbf{Yes or No}} & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark \\ 
\midrule
\textbf{Accuracy}    & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

